Enhancing Speaking Styles in Conversational Text-to-Speech Synthesis with Graph-based Multi-modal Context Modeling

Comparing with traditional text-to-speech (TTS) systems, conversational TTS systems are required to synthesize speeches with proper speaking style confirming to the conversational context. However, state-of-the-art context modeling methods in conversational TTS only model the textual information in context with a recurrent neural network (RNN). Such methods have limited ability in modeling the inter-speaker influence in conversations, and also neglect the speaking styles and the intra-speaker inertia inside each speaker. Inspired by DialogueGCN and its superiority in modeling such conversational influences than RNN based approaches, we propose a graph-based multi-modal context modeling method and adopt it to conversational TTS to enhance the speaking styles of synthesized speeches. Both the textual and speaking style information in the context are extracted and processed by DialogueGCN to model the inter- and intra-speaker influence in conversations. The outputs of DialogueGCN are then summarized by attention mechanism, and converted to the enhanced speaking style for current utterance. An English conversation corpus is collected and annotated for our research and released to public. Experiment results on this corpus demonstrate the effectiveness of our proposed approach, which outperforms the state-of-the-art context modeling method in conversational TTS in both MOS and ABX preference rate.

==> content/abstract2.tex <==
\begin{abstract}
%With the development of deep learning, 
%neural network based 
%text-to-speech (TTS) systems
%have shown their superiority than conventional TTS systems with fixed spoken style.
%and have been applied in many 
%human-computer conversational interaction scenarios.
%But
For conversational  
text-to-speech (TTS) systems,
%such as virtual assis-tants and chat bots, 
it is vital that the systems can adjust the spoken styles of synthesized speech according to different content and spoken styles in history conversations.
%synthesizing responses with reading style is unnatural in the conversational scenarios. 
%The spoken styles of the current speech are influenced by the historical conversations.
However, the study about learning spoken styles from history conversations
is still in its infancy.
Only the transcripts of the history conversations are considered, 
which neglects the spoken styles in history speeches.
%which also influence spoken style of the current sentence. 
Moreover, only the interactions of the global aspect between speakers are modeled, missing the party aspect self interactions inside each speaker.
%which is also re also proved to be highly related to the state of the current speaker.
%are still at very early stage. 
%However, most of these TTS systems 
%In conversations,
%spoken styles not only are used to express the intention, personality and state of the speaker,
%but also
%influence to
%the other participants in the conversations to choose proper
%spoken styles to response to such intention, personality and state.
%Such influence is cruel to intelligent human-computer conversational interaction
%and should be modelled in conversational TTS systems.
%are influenced
%by the personalities and states of each
%via their spoken style in speech
%which contains both social and personal attributes.
%These attributes are influencing the expressions of the following conversations and should be
%are 
%cruel to understand the purpose
%of users and generate natural responses.  
%Moreover, these systems only model the global conversation sequence.
%The sequences of the speeches of each speaker are also helpful to synthesize natural speeches. 
%To address this problem, 
In this paper,
to achieve better spoken style learning for conversational TTS,
we propose a spoken style learning approach
with multi-modal context encoding.
% for conversational TTS.
The textual information and spoken styles in the history conversations are 
processed 
through multiple hierarchical recurrent neural networks
to learn the spoken style related features
in global and party aspects.
The attention mechanism is further employed to summarize
these features
%which are most related to the current sentence
into a conversational context encoding.
%The spoken style of the current sentence is learnt from both the textual and spoken style information in historical conversations via hierarchical recurrent neural networks (RNNs) and attention mechanism.
%The historical information are modelled by the RNNs in global and per-participant aspects then summarized by 
Experimental results 
%on a spontaneous conversational corpus
demonstrate the effectiveness of our proposed approach, which outperform a baseline method using context encoding learnt only from the transcripts in global aspects,
with
MOS score on the naturalness of synthesized speech increasing from 3.138 to 3.408 and
ABX preference rate exceeding the baseline method by 36.45\%.
%show that our proposed method outperforms non-conversational TTS systems and other conversational TTS systems, 
%re used to
%Speaker-independent spoken style information is extracted from real conversations.
%the global and personal states of conversations
%via hierarchical recurrent neural networks.
\end{abstract}

==> content/abstract3.tex <==
\begin{abstract}
%With the development of deep learning, 
%neural network based 
%text-to-speech (TTS) systems
%have shown their superiority than conventional TTS systems with fixed spoken style.
%and have been applied in many 
%human-computer conversational interaction scenarios.
%But
%such as virtual assis-tants and chat bots, 
Comparing with traditional text-to-speech (TTS) systems,
conversational TTS systems are required to synthesize speeches with proper prosody matching the contexts.
%according to the content and spoken styles information in context.
%it is vital that the systems can 
%synthesizing responses with reading style is unnatural in the conversational scenarios. 
%The spoken styles of the current speech are influenced by the historical conversations.
However, the state-of-the-art studies on context modeling in conversational TTS
still use a single recurrent neural network to model the inter-speaker influence in conversation.
Such approaches neglect not only the acoustic information in contexts,
but also the intra-speaker influence in conversations.
Inspired by DialogueGCN and its ability in modeling conversational data,
%which also influence spoken style of the current sentence. 
%which is also re also proved to be highly related to the state of the current speaker.
%are still at very early stage. 
%However, most of these TTS systems 
%In conversations,
%spoken styles not only are used to express the intention, personality and state of the speaker,
%but also
%influence to
%the other participants in the conversations to choose proper
%spoken styles to response to such intention, personality and state.
%Such influence is cruel to intelligent human-computer conversational interaction
%and should be modelled in conversational TTS systems.
%are influenced
%by the personalities and states of each
%via their spoken style in speech
%which contains both social and personal attributes.
%These attributes are influencing the expressions of the following conversations and should be
%are 
%cruel to understand the purpose
%of users and generate natural responses.  
%Moreover, these systems only model the global conversation sequence.
%The sequences of the speeches of each speaker are also helpful to synthesize natural speeches. 
%To address this problem, 
%in this paper,
%to achieve better spoken style learning for conversational TTS,
we propose a conversational TTS approach
with graph-based multi-modal context modeling.
Both the text and speaker-independent acoustic information and in the contexts are extracted and processed 
by DialogueGCN %graph convolutional network
to learn the inter- and intra-speaker influence in conversation.
The outputs of DialogueGCN is weighted summed to a context encoding by attention mechanism,
then converted to predicted acoustic information for current sentence and synthesized to speech with proper prosody.
We collect and annotate a public English conversation corpus to support our research.
%which are most related to the current sentence
%The spoken style of the current sentence is learnt from both the textual and spoken style information in historical conversations via hierarchical recurrent neural networks (RNNs) and attention mechanism.
%The historical information are modelled by the RNNs in global and per-participant aspects then summarized by 
Experimental results 
%on a spontaneous conversational corpus
demonstrate the effectiveness of our proposed approach, 
with
MOS score on the naturalness of synthesized speech increasing from 3.356 to 3.584 and
ABX preference rate exceeding by 32.19\%
than a baseline approach with state-of-the-art context modeling method in conversational TTS.
%show that our proposed method outperforms non-conversational TTS systems and other conversational TTS systems, 
%re used to
%Speaker-independent spoken style information is extracted from real conversations.
%the global and personal states of conversations
%via hierarchical recurrent neural networks.
\end{abstract}

==> content/figure.tex <==
\begin{figure*}[t]
	\centering
	\begin{minipage}[b]{0.59\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/proposed.png}
		(a) Spoken style learning with multi-model hierarchical context encoding\\
		\includegraphics[width=.65\linewidth]{figures/baseline1.png}\\
		(a) Baseline approach
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.37\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/gst.png}
		(b) Speaker-independent GST-FastSpeech 
		\\\text{}\\
		\includegraphics[width=\linewidth]{figures/tts.png}
		(c) Conversational TTS framework
	\end{minipage}	\caption{
	    (a) Architecture of the proposed spoken style learning method with multi-model hierarchical context encoding. %for conversational TTS.
	    (b) Architecture of the speaker-independent global style token enhanced Tacotron framework.
	    (c) Architecture of the conversational TTS framework.
	}
	\label{fig:structure}
\end{figure*}

==> content/introduction2.tex <==
\section{Introduction}
%Toward intelligent human-robot speech interaction,
%text-to-speech (TTS) systems
%are required to understand the global 

%现有的reading style 的TTs已经做的很好了。
%   Tacotron blahblah
%   啥啥啥blahblah
% 
%converstaional TTS 而言，需要注重合成句子的prosody which 受上下文的内容与说话风格影响。
%对于口语对话交互而言，单纯reading style的合成反馈存在很大的不自然，亟需符合对话交互上下文的具有对话风格的语音（conversational TTS）合成。
% 已有工作对 conversational TTS进行了探索性的研究，这篇工作。。。。
%   讲课：上下文的内容是deep interaction。
%   一种conversational TTS 被提出， 利用上下文文本信息建模。
%   dialog rnn被提出，通过global 和party 两个方面来建模。
%
%但是，现在的 conversational TTS 没有充分利用语音信息。
%   对话交互语音信息中包含 social signal，会影响到说话的语气、情感，以及重音。
%   举例说明 social signal 对当前要合成的句子有影响。
%       Formal 的表达方式会希望对方也用formal的表达方式。
%       严肃的表达方式会希望对方也用严肃的表达方式。
% 亟需对对话交互中上述和social signal有关的acoustic attributs进行建模，并将其引入到conversational TTS的合成框架中。
% GST提供了一种控制合成语音风格的机制，取得了非常大的成功。基于此，本文希望通过类似GST的机制对social signal related acoustic attributes进行建模，并控制合成语音的分类（？）。
%   gst被提出用来建模说话方式（非文本信息）。
%
%为了利用语音信息，

With the development of deep learning,
neural network based text-to-speech (TTS) systems 
have achieved superior performance
%in speech synthesis 
%with a fixed spoken style 
than conventional TTS systems \cite{wang_tacotron:_2017, shen_natural_2017, gibiansky_deep_2017, miao_flow-tts_2020}.
However, they usually generate synthesized speech with a fixed spoken style.
While
%But %for conversational interaction systems such as 
for
%conversational TTS systems which are commonly used in 
conversational TTS systems with high levels of social ability \cite{vinciarelli_open_2015},
%such as virtual assistants and chat bots,
%synthesizing responses with reading style is unnatural % 不是很好 
it is vital that the systems can adjust the spoken styles of synthesized speech
according to %the details in the actual 
different contents and spoken styles in historical conversations.
In human-human conversations,
people are interacting with different social signals such as humor, empathy and compassion \cite{vinciarelli_open_2015}
through the contents and spoken styles in their speeches.
%In particular,
%people are producing social signals through their 
%replies and spoken styles 
%and expecting proper social signals from the replies and spoken styles produced by the other speakers. 
Therefore, 
for conversational TTS systems with given contents,
learning spoken styles from textual information and spoken styles in historical conversations is of great significance for realizing more natural human-computer speech interactions.
%and they are related and influenced by both the textual 
%and acoustic features in the historical conversations.
%and the other acoustic attributes in the historical speeches such as the spoken styles of each speaker.
%The historical conversations contain both the textual information in the 
%and the user attributes analysed from the user's speech.
%These details including the historical conversations
%in such conversational scenarios.
% TODO 过渡
% 引出 conversation tts 的特点，不能reading 需要 conversational ? style
% 需要考虑的因素，上下文
%the spoken styles used in the conversations are influenced by the conversation context.
%take place in highly specific contexts where people typically have a long history of previous relations \cite{vinciarelli_open_2015}.
%Therefore, learing spoken styles from the historical conversations
%historical conversations are vital to learn the proper spoken style to improve the prosody of synthesized speech.

However, such study of learning spoken styles from the historical conversations for conversational TTS systems is still in its early stage.
% TODO prosody 改 spoken style 与前文对应
Recently, 
%to improve the prosody in conversational TTS,
a conversational context encoder \cite{guo_conversational_2020} was proposed to 
learn a historical embedding from the historical conversations and adjust the spoken styles for conversational TTS by
processing the sentence embeddings of historical conversations through a uni-direction gated recurrent unit (GRU) \cite{cho_learning_2014} network.
This approach only deals with textual features in historical conversations,
neglecting
the spoken styles in historical dialogue.
Moreover, 
only
the global states \cite{majumder_dialoguernn_2019}
which model the interactions between different speakers 
are considered in this approach.
However, the party states \cite{majumder_dialoguernn_2019} which model the self interactions inside each speaker are also proved to be highly related to the state of the current speaker, are not considered.
%The party states \cite{majumder_dialoguernn_2019} which model the self interactions inside each speaker are also proved to be highly related to the state of the current speaker.

%These acoustic features such as the spoken styles
%are highly correlated with social signals such as 
%which are producing and expecting by people during communications \cite{vinciarelli_open_2015}.
% TODO: 改进一下说法
% 要引出spoken style
%Many social signals
%such as
% 提及一下 global 和 party
%Such expectations of social signals should be responded by conversational TTS systems 
%%based on the social signals in the historical 
%by modelling the related acoustic attributes in historical speeches.
% TODO 挪related works
%Global style token (GST) \cite{wang_style_2018} is proposed to unsupervisely learn the non-textual information of speeches as different spoken styles.

In this paper,
in order to improve the spoken style learning for conversational TTS,
we propose a spoken style learning method with multi-modal hierarchical context encoding.
% TODO: 加一句话
%to learn the spoken style of synthesized speech
%from both the textual and acoustic information in historical speeches 
%Pre-trained word embeddings \cite{song_directional_2018} are used as the textual information in the conversations.
%Then the sequence of word embeddings of a sentence is encoded by an encoder based on the encoder of Tacotron \cite{wang_tacotron:_2017}.
Global style token (GST) \cite{wang_style_2018} weights are extracted 
by a pre-trained multi-speaker GST enhanced Tacotron \cite{wang_tacotron:_2017} system (hereafter, GST-Tacotron)
in a speaker independent manner and used
as the ground-truth spoken styles for 
the
utterances in conversations.
%Speaker-independent GSTs are extracted as the ground-truths for the spoken styles in conversations.
Then the sentence level content embeddings 
in the textual domain
and the GST weights 
in the acoustic domain
in historical dialogue are used
to learn the spoken style related features
%to predict the GST of the current sentence
through multiple hierarchical bidirectional GRUs
consisting of a global bidirectional GRU and a party bidirectional GRU, aiming to respectively model the global and self interactions in the conversation.
Attention mechanism \cite{vaswani_attention_2017} is further used to summarize
the features that are most relevant to the current sentence from
the output of the hierarchical bidirectional GRUs into historical context encodings.
Then the historical context encodings are used to predict the GST weights of the current sentence.
The encoder, decoder and GST table in
the GST-Tacotron 
and the proposed spoken style learning model
form
our final conversational TTS framework. 
By giving the text and 
historical conversations,
%predicted GST weights of the current sentence,
the conversational TTS framework 
predicts the GST of the current sentence from the historical conversations
%with pre-trained GST tables,
%converts the 
%%predicted GST weights 
%historical conversations
%into GST of the current sentence %%with pre-trained GST tables,
and synthesizes the speech using the pre-trained encoder and decoder.

Experimental results
in both objective and subjective evaluations
on a spontaneous conversational corpus
demonstrate the effectiveness of our proposed method over
the baseline approach using context encoding that is learnt from transcripts only in global aspects.
The
MSE of the predicted GST weights decreasing from 
$3.17 \times 10^{-4}$ to $2.86 \times 10^{-4}$,
MOS score on the naturalness of the synthesized speech increasing from 3.138 to 3.408
and ABX rate on the naturalness of synthesized speech exceeding the baseline by 36.45\%.
The effectiveness of the multi-model information and the hierarchical architecture are also explored and demonstrated through ablation studies.
%and the GST of the historical conversations are concatenated and modelled through

%historical conversations
%textual and acoustic
%global and party aspects

%A speaker-independent GST learning network is proposed to exact the GSTs of the speeches in the conversations.
%Then the encoded textual information and the GST of the historical conversations are concatenated and modelled through
%hierarchical recurrent neural networks (RNNs) in global and party aspects.
%to predict the GST of the syntheized speech.

%which is most relative to the current sentence.

%The spoken style of the current sentence is learnt from both the textual and spoken style information in historical conversations via 
%The historical information are modelled by the RNNs




%show that our proposed method outperforms non-conversational TTS systems and transcript based conversational TTS systems in 
%re used to
%Speaker-independent spoken style information is extracted from real conversations.
%the global and personal states of conversations
%via hierarchical recurrent neural networks.
%not taking full advantages of the textual and spoken style information in 
%still directly using non-conversational TTS systems or primary conversational TTS systems which only process the transcripts of historical conversations.
%The spoken styles used in con

%such  context and the styles used in the context.
%directly applying these TTS systems in 
%will lead to unnatural response to users due to

%need more prosody

%speech processing,
%conversational interaction systems,
%are having more applications in daily use.
%To bring better user experience during interactions,
%conversational systems are hiring 
%due to their superiority in 
%These TTS systems are developed on encoder-decoder structure \cite{cho_learning_2014},
%using encoder to produce linguistic encodings and decoder to directly generate raw spectrogram.

%For conversational TTS systems,

%Moreover, the spoken styles used in historical conversations are also important for conversational TTS systems.
%Different Spoken styles are used to express the social signals and attributes of the speaker such as 
%Spoken styles contain 
%However, most of these TTS systems only process the transcripts of conversations,
%ignoring the spoken styles used in speeches.
%In conversations,
%spoken styles not only are used to express the intention, personality and state of the speaker,
%but also
%influence to
%the other participants in the conversations to choose proper
%spoken styles to response to such intention, personality and state.
%Such influence is cruel to intelligent human-computer speech interaction
%and should be modelled in conversational TTS systems.
%To synthesize natural speech to user,
%To modelling the deep interaction \cite{vinciarelli_open_2015} in conversations,
%Differing from non-conversational TTS systems,
%conversational TTS systems need to learn an internal representation from the historical conversations
%to further improve the prosody of the synthesized speech.
%and have been widely applied in conversational systems.

%are influenced
%by the personalities and states of each
%via their spoken style in speech
%which contains both social and personal attributes.
%These attributes are influencing the expressions of the following conversations and should be 
%are 
%cruel to understand the purpose
%of users and generate natural responses.  
%Moreover, these systems only model the global conversation sequence.
%The sequences of the speeches of each speaker are also helpful to synthesize natural speeches. 

%The rest of the paper is organized as follows.
%Section \ref{related} introduces the works that are highly related to our research.
%Section \ref{methodology} introduces the details of our purposed multi-modal hierarchical context encoding method.
%In Section \ref{experiments}, we describe our experiments and post the experimental results.
%Then conclusions and future directions are discussed in Section \ref{conclusions}.
%Finally in Section \ref{acknowledgements}, we thank the groups and sponsors for helping us with our research.

==> content/introduction3.tex <==
\section{Introduction}
With the development of deep learning,
neural network based text-to-speech (TTS) systems 
have achieved superior performance
%in speech synthesis 
%with a fixed spoken style 
than conventional TTS systems \cite{wang_tacotron:_2017, shen_natural_2017, gibiansky_deep_2017, miao_flow-tts_2020}.
However, 
for conversational TTS systems 
such as virtual assistants and voice agents,
%But %for conversational interaction systems such as 
%conversational TTS systems which are commonly used in 
%synthesizing responses with reading style is unnatural % 不是很好 
it is vital that the systems can synthesize speeches with proper prosody according to both the textual and acoustic information in contexts.
Moreover,
it is necessary for conversational systems to model both the inter- and intra-speaker dependency in contexts to  
understand how speakers influence the emotional states of each other and the emotional inertia inside themselves \cite{}.

%and they are related and influenced by both the textual 
%and acoustic features in the historical conversations.
%and the other acoustic attributes in the historical speeches such as the spoken styles of each speaker.
%The historical conversations contain both the textual information in the 
%and the user attributes analysed from the user's speech.
%These details including the historical conversations
%in such conversational scenarios.
% TODO 过渡
% 引出 conversation tts 的特点，不能reading 需要 conversational ? style
% 需要考虑的因素，上下文
%the spoken styles used in the conversations are influenced by the conversation context.
%take place in highly specific contexts where people typically have a long history of previous relations \cite{vinciarelli_open_2015}.
%Therefore, learing spoken styles from the historical conversations
%historical conversations are vital to learn the proper spoken style to improve the prosody of synthesized speech.

However, the context modeling methods in state-of-art conversational TTS systems are still in their early stage.
Most recent work propose a conversational context encoder \cite{guo_conversational_2020} to 
learn a context embedding by sequentially processing the sentence embeddings of historical conversations through a uni-direction gated recurrent unit (GRU) \cite{cho_learning_2014} network.
This approach only deals with textual features in historical conversations,
neglecting the acoustic information in speeches.
Moreover, 
such recurrent neural network (RNN) based method only model the inter-speaker dependency in conversations,
and hard to model intra-speaker dependency.

%The party states \cite{majumder_dialoguernn_2019} which model the self interactions inside each speaker are also proved to be highly related to the state of the current speaker.

%These acoustic features such as the spoken styles
%are highly correlated with social signals such as 
%which are producing and expecting by people during communications \cite{vinciarelli_open_2015}.
% TODO: 改进一下说法
% 要引出spoken style
%Many social signals
%such as
% 提及一下 global 和 party
%Such expectations of social signals should be responded by conversational TTS systems 
%%based on the social signals in the historical 
%by modelling the related acoustic attributes in historical speeches.
% TODO 挪related works
%Global style token (GST) \cite{wang_style_2018} is proposed to unsupervisely learn the non-textual information of speeches as different spoken styles.

Inspired by the superiority of DialogueGCN \cite{} in modelling both the inter- and intra-speaker influences
than RNN based approaches,
we propose a conversational TTS approach with graph-based multi-model context encoding.
Both the textual and acoustic information in the contexts are extracted by a sentence level content encoder and a 
global style token (GST) \cite{wang_style_2018} enhanced multi-speaker FastSpeech \cite{} model (hereafter, GST-FastSpeech).
DialogueGCN is then employed to learn the influences in conversations and 
attention mechanism \cite{vaswani_attention_2017} is then used to summarize
%the features that are most relevant to the current sentence from
the output of the DialogueGCN into context encodings.
The context encodings is then converted to predicted acoustic information for the current sentence
and synthesize to speech with proper prosody by the previous GST-FastSpeech2.

We collect and annotate an English conversation corpus for our research.
And experimental results in both objective and subjective evaluations demonstrate the effectiveness of our proposed method over
the baseline approach with RNN based context modeling method.
The mean squared error (MSE) of the predicted GST weights decreasing from 
$5.15 \times 10^{-3}$ to $4.17 \times 10^{-3}$,
MOS score on the naturalness of the synthesized speech increasing from 3.356 to 3.584
and ABX rate on the naturalness of synthesized speech exceeding the baseline by 32.19\%.
The effectiveness of the proposed graph-based multi-model context encoding method are also explored and demonstrated through ablation studies.
%and the GST of the historical conversations are concatenated and modelled through

%historical conversations
%textual and acoustic
%global and party aspects

%A speaker-independent GST learning network is proposed to exact the GSTs of the speeches in the conversations.
%Then the encoded textual information and the GST of the historical conversations are concatenated and modelled through
%hierarchical recurrent neural networks (RNNs) in global and party aspects.
%to predict the GST of the syntheized speech.

%which is most relative to the current sentence.

%The spoken style of the current sentence is learnt from both the textual and spoken style information in historical conversations via 
%The historical information are modelled by the RNNs




%show that our proposed method outperforms non-conversational TTS systems and transcript based conversational TTS systems in 
%re used to
%Speaker-independent spoken style information is extracted from real conversations.
%the global and personal states of conversations
%via hierarchical recurrent neural networks.
%not taking full advantages of the textual and spoken style information in 
%still directly using non-conversational TTS systems or primary conversational TTS systems which only process the transcripts of historical conversations.
%The spoken styles used in con

%such  context and the styles used in the context.
%directly applying these TTS systems in 
%will lead to unnatural response to users due to

%need more prosody

%speech processing,
%conversational interaction systems,
%are having more applications in daily use.
%To bring better user experience during interactions,
%conversational systems are hiring 
%due to their superiority in 
%These TTS systems are developed on encoder-decoder structure \cite{cho_learning_2014},
%using encoder to produce linguistic encodings and decoder to directly generate raw spectrogram.

%For conversational TTS systems,

%Moreover, the spoken styles used in historical conversations are also important for conversational TTS systems.
%Different Spoken styles are used to express the social signals and attributes of the speaker such as 
%Spoken styles contain 
%However, most of these TTS systems only process the transcripts of conversations,
%ignoring the spoken styles used in speeches.
%In conversations,
%spoken styles not only are used to express the intention, personality and state of the speaker,
%but also
%influence to
%the other participants in the conversations to choose proper
%spoken styles to response to such intention, personality and state.
%Such influence is cruel to intelligent human-computer speech interaction
%and should be modelled in conversational TTS systems.
%To synthesize natural speech to user,
%To modelling the deep interaction \cite{vinciarelli_open_2015} in conversations,
%Differing from non-conversational TTS systems,
%conversational TTS systems need to learn an internal representation from the historical conversations
%to further improve the prosody of the synthesized speech.
%and have been widely applied in conversational systems.

%are influenced
%by the personalities and states of each
%via their spoken style in speech
%which contains both social and personal attributes.
%These attributes are influencing the expressions of the following conversations and should be 
%are 
%cruel to understand the purpose
%of users and generate natural responses.  
%Moreover, these systems only model the global conversation sequence.
%The sequences of the speeches of each speaker are also helpful to synthesize natural speeches. 

%The rest of the paper is organized as follows.
%Section \ref{related} introduces the works that are highly related to our research.
%Section \ref{methodology} introduces the details of our purposed multi-modal hierarchical context encoding method.
%In Section \ref{experiments}, we describe our experiments and post the experimental results.
%Then conclusions and future directions are discussed in Section \ref{conclusions}.
%Finally in Section \ref{acknowledgements}, we thank the groups and sponsors for helping us with our research.

==> content/methodology2.tex <==
\section{Methodology}
\label{methodology}

As shown in Figure \ref{fig:structure},
our work consists of three parts.
In Section \ref{style learning}, we introduce our proposed spoken style learning method with multi-model hierarchical context encoding for conversational TTS.
The ground-truth GST weights are extracted from a speaker-independent GST-Tacotron model which we will describe in Section \ref{gst}.
%In this section, we will firstly introduce our proposed multi-modal hierarchical context encoding for spoken style learning in conversational TTS.
%Then we will introduce the speaker-independent GST learning network to extract the GSTs which are used as the features and labels in spoken style learning in conversational TTS.
Then the encoder, decoder and GST table in GST-Tacotron 
and our proposed spoken style learning model
form our final conversational TTS framework which is shown in Figure \ref{fig:structure}(c).
%we will describe in Section \ref{conversational TTS}. 
By giving the text of the current sentence and 
historical conversations,
%predicted GST weights of the current sentence,
the spoken style learning part
predicts the GST weights from the historical conversations.
The GST weights
are further converted to the GST of the current sentence 
with the pre-trained GST table.
Then the encoder and decoder in the GST-Tacotron synthesizes speech with the predicted GST and the given speaker embedding.


\subsection{Spoken style learning with graph-based multi-modal context encoding in conversational TTS}
\label{style learning}
To model the spoken style related features from the content and spoken styles in historical conversations in both global and party aspects,
we propose a spoken style learning approach
with multi-modal hierarchical context encoding.
%Inspired by DialogueRNN \cite{majumder_dialoguernn_2019}
%we proposed a hierarchical network to model the deep interactions in conversations from both the textual and acoustic information in historical conversations.
%in both global and party aspects.

As shown in Figure \ref{fig:structure}(a), 
the transcripts of the historical conversations are converted to word embeddings by a pre-trained word embedding model \cite{song_directional_2018}.
%and used as the textual information of historical conversations.
%the inputs for the textual information of historical conversations are word embeddings.
% TODO: 为什么To 
%We employ pre-trained word embeddings \cite{song_directional_2018} which are trained from a carefully designed corpus which have good coverage, freshness, and accuracy on spontaneous conversations.
% TODO: 可能得改，再议
Then a sentence level content encoder is used to encode the word embeddings into 
content embedding for each sentence.
The content encoder consists of a pre-net and a CBHG network \cite{lee_fully_2017}.
%content embeddings for each sentence, which consists of a pre-net and a CBHG network \cite{lee_fully_2017}.
The pre-net consists of two fully connected layers which have 128 and 256 hidden units respectively with dropout probability 0.5.
The CBHG network has the same structure with the CBHG network used in Tacotron \cite{wang_tacotron:_2017}, which consists of a bank of 1-D convolutional filters, a max pooling layer, four highway networks \cite{srivastava_highway_2015} and a bidirectional GRU network.
% TODO: 得改
After encoding, the output of the last step in the bidirectional GRU network
is used as the content embedding of a given sentence.

% To 加入 acoustic feature, 为什么要用GST
% GST是一种很好的表征
We employ GST weights as the spoken style information of historical speeches.
The GST weights are extracted by a GST weight extractor trained in a speaker-independent GST-Tacotron model which we will describe in Section \ref{gst}.
%During inference and real human-computer conversational scenarios,
%instead of re-extracting GSTs from the speeches synthesized by the computer,
%we can directly use the predicted GSTs of the synthesized speeches as inputs.

Sentence embeddings which are the concatenation of the content embeddings and the GST weights for each sentence are used as the inputs for the following hierarchical networks.
%Three kinds of bidirectional GRU are hierarchically stacked to model the global and self interactions and learn spoken style related features in conversations, which all have 256 hidden units and dropout rate 0.9.
%The global bidirectional GRU takes the concatenated sentence embeddings of 
%the historical conversations 
%as inputs to model the interactions between the participants in the conversation.
%The outputs of the global bidirectional GRU are masked for each participant, resulting in multiple masked output sequences.
%In detail, for each participant, the outputs of the sentence spoken by the other participants are masked to zero.
%Party bidirectional GRU is used for each participant
%to model the self interactions inside each participant from the corresponding masked sequence.
%Then the outputs of party bidirectional GRU for each participant are concatenated and processed by the style learning bidirectional GRU to learn the spoken style related features in historical conversations.
%The above procedures can also be formulated as the following equations:
%\begin{align}
%  O^G &= BiGRU^G(S) \\
%  %O^M_i &= O^G \odot Mask_i \\
%  O^P_i &= BiGRU^P(O^G \odot Mask_i) \\
%  O^P &= [O^P_1, \dots ,O^P_N] \\
%  O^S &= BiGRU^S(O^P)
%\end{align}
%where $S$ is the concatenated sentence embeddings of the historical conversations,
%$BiGRU^{\{G,P,S\}}$ are the global, party and style learning bidirectional GRU respectively,
%$O^G$ is the outputs of the global bidirectional GRU,
%$i$ is the $i$-th participant in the conversation,
%$Mask_i$ is a binary matrix in which only the elements that belong to the sentences spoken by the $i$-th participant are set to 1,
%%$O^M_i$ is the masked sequences of the global GRU for participant $i$,
%$O^P_i$ is the outputs of the party bidirectional GRU for the $i$-th participant,
%$O^P$ is the concatenation of the outputs of the party bidirectional GRU for all $N$ participants
%%$N$ is the number of participants,
%and $O^S$ is the output of the style learning bidirectional GRU.

The attention mechanism \cite{vaswani_attention_2017} is further used to summarize
the features that are most relevant
to the current sentence.
%from the output of the hierarchical bidirectional GRUs into a historical context encoding to predict the GST weights of the current sentence.
% TODO: 说明一下为什么用这个做query
The content embedding of the current sentence and
the one-hot label of the current speaker 
are concatenated as the sentence embedding of the current sentence.
The relations between the sententce embedding of the current sentence 
and the outputs of the style learning bidirectional GRU are calculated 
by the additive attention mechanism \cite{bahdanau_neural_2014} 
as attention weights.
%is used as the query for the attention mechanism.
%Then the attention weights of each historical sentences are calculated 
Then the outputs of the style learning bidirectional GRU are weighted summed into a conversational context embedding with the attention weights.

The sentence embedding of the current sentence and the conversational context embedding are then concatenated and projected to GST weights.
A fully connected layer
with dropout probability 0.5
is used for the projection.

The mean squared error (MSE)
between the predicted and ground-truth GST weights
is used as the loss function for our proposed spoken style learning approach.

%of each utterance from interactive context information 
%the corresponding participant produced by

\subsection{Speaker-independent global style token learning}
\label{gst}

GST \cite{} is proposed for Tacotron \cite{wang_style_2018} (here after, GST-Tacotron) to unsupervisely learn the non-textual information in speeches as different spoken styles.
However, the speaker information is not seperated from GST in the original GST-Tacotron framework.
Moreover, GST-Tacotron may fail to synthesize speech with GST tranferred from another speech.
%the extracted GSTs may fail to be transferred to by GST-Tacotron due to the robustness of Tacotron.
Inspired by the effectiveness and robustness of FastSpeech \cite{},
we proposed an speaker-independent GST learning framework for FastSpeech (here after, GST-FastSpeech).
%may also embed speaker information into GSTs for conversations with multiple speakers. 
%To improve the , we 
%To 
%proactively discourage the GSTs from also capturing speaker information
%%address this problem and achieve robust GST learning 
%in the conversational scenarios,
%we propose a speaker-independent GST learning method based on the original GST-Tacotron.

%\begin{figure}[htb]
%  \centering
%  \includegraphics[width=.8\linewidth]{figures/gst.png}
%  \caption{Structure of the speaker-independent global style token learning framework.}
%  \label{fig:gst}
%\end{figure}

As shown in Figure \ref{fig:structure}(b),
we introduce the reference encoder and the style token attention from the original GST-Tacotron
with domain adversarial training \cite{ganin_domain-adversarial_2016} to 
learing GST and separate speaker information in GST-FastSpeech.

encourage the framework to encode GSTs in a speaker-independent manner
the speaker-independent module 
most parts of the model are same to those in the 

The GST of speech is represented as a weighted average of the GST bases in the GST table
through a reference encoder and attention mechanism.
Based on the original GST-Tacotron, we further employ 
by introducing a speaker identifier based on the GST and 
a gradient reversal layer \cite{ganin_domain-adversarial_2016}.
The speaker identifier consists of a single fully connected layer and tries to predict the ground-truth speaker embeddings which are x-vectors \cite{snyder_x-vectors_2018} extracted by a pre-trained model from GSTs.
The gradient reversal layer is inserted prior to the speaker identifier with weight -0.1.
To recover the speech from the speaker-independent GST,
the ground-truth speaker embedding are used as an additional input for the decoder.
The MSE between the predicted and ground-truth x-vectors is used as an additional adversarial loss function.

After trained, the
reference encoder and attention mechanism for GST learning form the GST weight extractor for our proposed spoken style learning framework.
And the encoder, decoder and GST table are transferred to the conversaional TTS framework.
%learnt speaker-independent GSTs is used as the acoustic features of the historcial speeches and the ground truth GST of the current speech. 
%During inference, the speaker-independent GST learning network is also used to synthesize responses to users with predicted GSTs.

==> content/related.tex <==
\section{Related works}
\label{related}

% TODO 再强reading style
For synthesizing speeches with fixed spoken style,
neural network TTS systems \cite{wang_tacotron:_2017, shen_natural_2017, gibiansky_deep_2017, miao_flow-tts_2020},
such as Tacotron \cite{wang_tacotron:_2017} and Tacotron 2 \cite{shen_natural_2017},
merge many components in conventional TTS systems into one trainable neural network,
not only saving time and resources during development,
but also bringing further improvements to the naturalness of the synthesized speech.
These systems are mainly developed in encoder-decoder \cite{cho_learning_2014} with attention \cite{bahdanau_neural_2014} structure, using encoder to produce linguistic encodings and decoder to generate spectrogram. 

However, few works are proposed in conversational TTS.
An end-to-end approach \cite{guo_conversational_2020} is proposed to learn the spoken styles from the transcripts of the historical conversations for voice agents.
% TODO: To blahblah
%An auxiliary encoder is proposed and added to a phoneme-based TTS system to add the textual information of the current sentence.
% TODO: To blahblha
In this approach, a conversational context encoder is also proposed to encode the sentence embeddings of historical conversations through a GRU.
This approach is missing the spoken styles in historical speeches which are related to the spoken style of the current sentence.
%However, 关于历史信息的应用上
%强调一下音频的作用
%强调一下party aspect的作用
And this approach is only considering the interactions of different speakers,
missing the self interactions inside each speakers.

% 虽然 TTS 少，但是
In modeling the historical information in the context, many algorithms are proposed and used in conversational speech emotion modelling \cite{majumder_dialoguernn_2019, lian_conversational_2020, shi_dimensional_2020} and other conversational applications \cite{atamna_hri-rnn_2020, fuscone_neural_2020, kim_speech_2020}.
DialogueRNN \cite{majumder_dialoguernn_2019}
is proposed to model the interactions in the conversations through multiple recurrent neural networks in both global and party aspects.
Graph neural networks are also employed to model the context-sensitive and speaker-sensitive dependencies in conversations \cite{lian_conversational_2020}.
And an dimentional emotion prediction network \cite{shi_dimensional_2020} is proposed to find the emotional state related features from both textual and acoustic features.

==> tables/ablation.tex <==
\begin{table}[tb]
  \caption{Objective evaluations for the variant approaches in ablation studies.}
  \label{tab:ablation}
  \centering
  \begin{tabular}{ccc}
    \toprule
    & \textbf{Variant 1} &\textbf{Variant 2} \\
    \midrule
    \textbf{MSE} & $2.96 \times 10^{-4}$ & $3.01 \times 10^{-4}$ \\
    \bottomrule
  \end{tabular}
\end{table}

==> tables/objective.tex <==
\begin{table}[htb]
  \caption{Objective evaluations for different approaches}
  \label{tab:objective}
  \centering
  \begin{tabular}{ccccc}
    \toprule
    &\textbf{Baseline} &\textbf{Proposed} &\textbf{Variant 1} &\textbf{Variant 2}\\
    \midrule
    \textbf{MSE ($10^{-3}$)} & 5.15 & \textbf{} & 2.96 & 3.01 \\
    \bottomrule
  \end{tabular}
\end{table}
